Temporal Representation Learning for Stock Similarities and Its Applications in Investment Management

In the era of rapid globalization and digitalization, accurate identification of similar stocks has become increasingly challenging due to the non-stationary nature of financial markets and the ambiguity in conventional regional and sector classifications. To address these challenges, we examine SimStock, a novel temporal self-supervised learning framework that combines techniques from self-supervised learning (SSL) and temporal domain generalization to learn robust and informative representations of financial time series data. The primary focus of our study is to understand the similarities between stocks from a broader perspective, considering the complex dynamics of the global financial landscape. We conduct extensive experiments on four real-world datasets with thousands of stocks and demonstrate the effectiveness of SimStock in finding similar stocks, outperforming existing methods. The practical utility of SimStock is showcased through its application to various investment strategies, such as pairs trading, index tracking, and portfolio optimization, where it leads to superior performance compared to conventional methods. Our findings empirically examine the potential of data-driven approach to enhance investment decision-making and risk management practices by leveraging the power of temporal self-supervised learning in the face of the ever-changing global financial landscape.

==> Tables/chap4_SNP500.tex <==
\fontsize{8}{9}\selectfont{
\begin{tabular}{r|cccc|cccc|cccc|cccc}
\hline
S\&P500 | 30 Stocks    & \multicolumn{4}{c|}{Target Volatility (24\%)} & \multicolumn{4}{c|}{Target Volatility (27\%)} & \multicolumn{4}{c|}{Target Volatility (30\%)} & \multicolumn{4}{c}{Target Volatility (33\%)} \\ \hline
Covariance Method      & SS        & HC        & SM        & GS        & SS        & HC        & SM        & GS        & SS        & HC        & SM         & GS       & SS        & HC        & SM        & GS       \\ \hline
Arithmetic Return (\%) & 11.31     & 10.04     & 9.61      & 10.14     & 12.22     & 10.75     & 11.02     & 11.05     & 12.84     & 11.66     & 12.03      & 11.97    & 13.33     & 12.50     & 12.85     & 12.69    \\ \cline{1-1}
Geometric Return (\%)  & 10.39     & 9.30      & 8.97      & 9.43      & 11.158    & 9.86      & 10.21     & 10.17     & 11.60     & 10.57     & 10.967     & 10.83    & 11.88     & 11.18     & 11.51     & 11.32    \\ \cline{1-1}
Cumulative Return (\%) & 37.36     & 33.07     & 31.60     & 33.40     & 40.54     & 35.40     & 36.63     & 36.49     & 42.64     & 38.44     & 39.930     & 39.61    & 44.18     & 41.27     & 42.59     & 42.05    \\ \cline{1-1}
Annualized SD (\%)     & 28.82     & 27.27     & 26.61     & 27.00     & 30.24     & 28.92     & 28.66     & 28.90     & 31.72     & 30.58     & 30.623     & 30.79    & 33.25     & 32.17     & 32.49     & 32.54    \\ \cline{1-1}
Annualized Skewness    & -0.12     & -0.15     & -0.12     & -0.122    & -0.14     & -0.17     & -0.16     & -0.16     & -0.18     & -0.20     & -0.191     & -0.20    & -0.22     & -0.22     & -0.22     & -0.23    \\ \cline{1-1}
Annualized Kurtosis    & 3.17      & 3.22      & 3.23      & 3.161     & 3.22      & 3.28      & 3.29      & 3.24      & 3.27      & 3.33      & 3.343      & 3.28     & 3.27      & 3.33      & 3.33      & 3.28     \\ \cline{1-1}
Maximum Drawdown (\%)  & -24.90    & -23.96    & -23.47    & -23.599   & -25.65    & -25.36    & -24.57    & -25.04    & -26.69    & -26.44    & -25.971    & -26.57   & -28.20    & -27.63    & -27.57    & -28.08   \\ \cline{1-1}
Monthly 95\% VaR (\%)  & -10.44    & -10.22    & -9.99     & -10.058   & -10.77    & -10.63    & -10.53    & -10.52    & -11.19    & -10.95    & -10.921    & -11.01   & -11.72    & -11.40    & -11.48    & -11.56   \\ \cline{1-1}
Sharpe Ratio           & 0.44      & 0.40      & 0.39      & 0.421     & 0.46      & 0.41      & 0.43      & 0.43      & 0.46      & 0.42      & 0.447      & 0.43     & 0.45      & 0.43      & 0.44      & 0.43     \\ \cline{1-1}
Annualized Turnover    & 8.68      & 8.39      & 8.49      & 8.361     & 8.69      & 8.48      & 8.56      & 8.49      & 8.73      & 8.54      & 8.592      & 8.56     & 8.67      & 8.57      & 8.51      & 8.54     \\ \cline{1-1}
Portfolio Wealth       & 137641    & 133514    & 131587    & 133197    & 140816    & 136640    & 136761    & 135554    & 143033    & 139817    & 140129     & 138665   & 144468    & 142346    & 142841    & 141557   \\ \hline
\end{tabular}}

==> Tables/chap4_TSE150.tex <==
\fontsize{8}{9}\selectfont{
\begin{tabular}{r|cccc|cccc|cccc|cccc}
\hline
JPX Prime 150 | 30 Stocks & \multicolumn{4}{c|}{Target Volatility (24\%)}                                                                      & \multicolumn{4}{c|}{Target Volatility (27\%)}                                                                       & \multicolumn{4}{c|}{Target Volatility (30\%)}                                                                      & \multicolumn{4}{c}{Target Volatility (33\%)}                                                                      \\ \hline
Covariance Method         & SS                         & HC                         & SM                         & GS                          & SS                         & HC                         & SM                          & GS                          & SS                         & HC                         & SM                         & GS                          & SS                         & HC                         & SM                         & GS                         \\ \hline
Arithmetic Return (\%)    & 20.12                      & 19.02                      & 18.61                      & 17.80                       & 20.85                      & 19.78                      & 20.02                       & 19.20                       & 21.70                      & 20.65                      & 21.40                      & 20.51                       & 22.47                      & 21.70                      & 22.50                      & 21.96                      \\ \cline{1-1}
Geometric Return (\%)     & 18.63                      & 17.72                      & 17.24                      & 16.62                       & 19.24                      & 18.31                      & 18.40                       & 17.78                       & 19.96                      & 19.01                      & 19.58                      & 18.90                       & 20.62                      & 19.90                      & 20.57                      & 20.14                      \\ \cline{1-1}
Cumulative Return (\%)    & 71.15                      & 66.53                      & 64.60                      & 61.55                       & 74.32                      & 69.56                      & 70.25                       & 67.23                       & 77.95                      & 73.23                      & 76.27                      & 72.90                       & 81.67                      & 77.87                      & 81.37                      & 79.30                      \\ \cline{1-1}
Annualized SD (\%)        & 26.83                      & 26.16                      & 25.56                      & 25.71                       & 28.51                      & 27.88                      & 27.74                       & 27.74                       & 29.99                      & 29.59                      & 29.83                      & 29.69                       & 31.33                      & 31.20                      & 31.59                      & 31.46                      \\ \cline{1-1}
Annualized Skewness       & 0.28                       & 0.16                       & 0.17                       & 0.13                        & 0.32                       & 0.17                       & 0.21                        & 0.18                        & 0.34                       & 0.19                       & 0.23                       & 0.21                        & 0.32                       & 0.19                       & 0.23                       & 0.20                       \\ \cline{1-1}
Annualized Kurtosis       & 3.37                       & 2.94                       & 2.99                       & 2.92                        & 3.43                       & 3.02                       & 3.08                        & 3.01                        & 3.49                       & 3.06                       & 3.17                       & 3.09                        & 3.51                       & 3.12                       & 3.22                       & 3.16                       \\ \cline{1-1}
Maximum Drawdown (\%)     & -19.17                     & -19.63                     & -19.52                     & -19.44                      & -20.37                     & -20.89                     & -20.85                      & -20.62                      & -21.16                     & -22.09                     & -22.15                     & -21.96                      & -22.19                     & -23.28                     & -23.29                     & -23.14                     \\ \cline{1-1}
Monthly 95\% VaR (\%)     & -8.52                      & -8.89                      & -8.49                      & -8.82                       & -9.00                      & -9.46                      & -9.20                       & -9.36                       & -9.41                      & -9.95                      & -9.79                      & -9.90                       & -9.79                      & -10.46                     & -10.31                     & -10.40                     \\ \cline{1-1}
Sharpe Ratio              & 0.96                       & 0.92                       & 0.91                       & 0.86                        & 0.93                       & 0.89                       & 0.90                        & 0.86                        & 0.92                       & 0.87                       & 0.90                       & 0.87                        & 0.92                       & 0.87                       & 0.90                       & 0.88                       \\ \cline{1-1}
Annualized Turnover       & 8.81                       & 8.38                       & 8.50                       & 8.54                        & 8.83                       & 8.52                       & 8.57                        & 8.62                        & 8.81                       & 8.59                       & 8.56                       & 8.59                        & 8.85                       & 8.58                       & 8.54                       & 8.54                       \\ \cline{1-1}
Portfolio Wealth          & \multicolumn{1}{r}{172884} & \multicolumn{1}{r}{161548} & \multicolumn{1}{r}{164604} & \multicolumn{1}{r|}{166538} & \multicolumn{1}{r}{177019} & \multicolumn{1}{r}{167221} & \multicolumn{1}{r}{170254.} & \multicolumn{1}{r|}{169561} & \multicolumn{1}{r}{181526} & \multicolumn{1}{r}{172900} & \multicolumn{1}{r}{176279} & \multicolumn{1}{r|}{173231} & \multicolumn{1}{r}{185350} & \multicolumn{1}{r}{179285} & \multicolumn{1}{r}{181366} & \multicolumn{1}{r}{177877} \\ \hline
\end{tabular}}

==> Tables/chap4_Tracking_EW_top_k.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\centering
\fontsize{6}{7}\selectfont{
\begin{tabular}{clccccc}
\hline
\multirow{2}{*}{\textbf{Query ETFs}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{5}{c}{\textbf{Top $k$ similar stocks}}                                                                                                    \\
                                 & \multicolumn{1}{c}{}                                  & \textbf{@1}                          & \textbf{@2}                       & \textbf{@3}          & \textbf{@4}                & \textbf{@5}           \\ \hline
\multirow{2}{*}{ARKK}            & SimStock                                              & Stratasys                            & Zuora                             & 3D Systems Corp      & Transaction Media Networks & Azenta                \\
                                 & Corr2                                                 & China Southern Power Grid Technology & BlackLine                         & Twist Bioscience     & Block                      & MercadoLibre          \\ \hline
\multirow{2}{*}{SKYY}            & SimStock                                              & ServiceNow                           & Guidewire Software                & Elastic N.V.         & Splunk                     & Intuit                \\
                                 & Corr2                                                 & China Southern Power Grid Technology & Electro Optic Systems             & Catalent             & Sea Limited                & IDEXX Laboratories    \\ \hline
\multirow{2}{*}{BOTZ}            & SimStock                                              & Pci Technology Group                 & Applied Materials                 & Seiko Corporation    & Zhejiang Taotao Vehicles   & Teradyne              \\
                                 & Corr2                                                 & China Southern Power Grid Technology & Artisan Partners Asset Management & Yeti Holdings        & Floor \& Decor Holdings     & Cognex Corporation    \\ \hline
\multirow{2}{*}{LIT}             & SimStock                                              & Livent Corp                          & Albemarle Corp                    & IQVIA Holdings Inc   & KKR \& Co                   & Trimble Inc           \\
                                 & Corr2                                                 & China Southern Power Grid Technology & Great Wall Motor Company Limited  & Sungrow Power Supply & BYD Company Limited        & Albemarle Corporation \\ \hline
\end{tabular}}


==> Tables/chap4_mv_30.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\fontsize{10}{11}\selectfont{
\begin{tabular}{rcccccccc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Evaluation Method}} & \multicolumn{8}{c}{MinVariance | 30 stocks}                                                \\ \cline{2-9} 
\multicolumn{1}{c}{}                                   & \multicolumn{4}{c}{S\&P500}                            & \multicolumn{4}{c}{JPX Prime 150} \\ \hline
\multicolumn{1}{r|}{Covariance Method}                 & SS     & HC     & SM     & \multicolumn{1}{c|}{GS}     & SS     & HC     & SM     & GS     \\ \hline
\multicolumn{1}{r|}{Arithmetic Return (\%)}            & 3.72   & 0.94   & -0.63  & \multicolumn{1}{c|}{0.11}   & 11.31  & 10.04  & 9.61   & 10.14  \\ \cline{1-1}
\multicolumn{1}{r|}{Geometric Return (\%)}             & 3.00   & 0.56   & -0.87  & \multicolumn{1}{c|}{-0.17}  & 10.39  & 9.30   & 8.97   & 9.43   \\ \cline{1-1}
\multicolumn{1}{r|}{Cumulative Return (\%)}            & 10.59  & 2.67   & -2.25  & \multicolumn{1}{c|}{-0.03}  & 37.36  & 33.07  & 31.60  & 33.40  \\ \cline{1-1}
\multicolumn{1}{r|}{Annualized SD (\%)}                & 22.48  & 19.14  & 16.40  & \multicolumn{1}{c|}{17.66}  & 28.82  & 27.27  & 26.61  & 27.00  \\ \cline{1-1}
\multicolumn{1}{r|}{Annualized Skewness}               & -0.02  & -0.17  & 0.11   & \multicolumn{1}{c|}{0.02}   & -0.12  & -0.15  & -0.12  & -0.12  \\ \cline{1-1}
\multicolumn{1}{r|}{Annualized Kurtosis}               & 2.56   & 3.12   & 2.98   & \multicolumn{1}{c|}{2.89}   & 3.17   & 3.22   & 3.23   & 3.16   \\ \cline{1-1}
\multicolumn{1}{r|}{Maximum Drawdown (\%)}             & -22.29 & -21.89 & -19.44 & \multicolumn{1}{c|}{-20.05} & -24.90 & -23.96 & -23.47 & -23.59 \\ \cline{1-1}
\multicolumn{1}{r|}{Monthly 95\% VaR (\%)}             & -8.87  & -7.97  & -7.20  & \multicolumn{1}{c|}{-7.51}  & -10.44 & -10.22 & -9.99  & -10.05 \\ \cline{1-1}
\multicolumn{1}{r|}{Sharpe Ratio}                      & 0.05   & -0.14  & -0.29  & \multicolumn{1}{c|}{-0.21}  & 0.44   & 0.40   & 0.39   & 0.42   \\ \cline{1-1}
\multicolumn{1}{r|}{Annualized Turnover}               & 1.17   & 7.05   & 5.47   & \multicolumn{1}{c|}{6.18}   & 8.68   & 8.39   & 8.49   & 8.36   \\ \cline{1-1}
\multicolumn{1}{r|}{Portfolio Wealth}                  & 110414 & 99935  & 97747  & \multicolumn{1}{c|}{102663} & 137641 & 133514 & 131587 & 133197 \\ \hline
\end{tabular}}


==> Tables/chap4_sim_qualitative.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{cccccccc}
\hline
\multicolumn{1}{l}{}                           &                           & \multicolumn{6}{c}{\textbf{First Trust Cloud Computing ETF (SKYY)}}                                                                                                                           \\
\multicolumn{1}{l}{\multirow{-2}{*}{Exchange}} & \multirow{-2}{*}{Methods} & \textbf{TOP@10}               & \textbf{TOP@15}               & \textbf{TOP@20}               & \textbf{TOP@25}               & \textbf{TOP@30}               & \textbf{TOP@35}               \\ \hline
                                               & corr1                     & {\color[HTML]{009901} 0.1150} & {\color[HTML]{009901} 0.1406} & {\color[HTML]{009901} 0.1379} & {\color[HTML]{009901} 0.1245} & {\color[HTML]{009901} 0.1058} & {\color[HTML]{009901} 0.0993} \\
                                               & corr2                     & 0.2410                        & 0.2298                        & 0.2011                        & 0.1916                        & 0.1586                        & 0.1455                        \\
                                               & TS2VEC                    & 0.1849                        & 0.1655                        & 0.1407                        & 0.1397                        & 0.1387                        & 0.1330                        \\
\multirow{-4}{*}{US}                           & SimStock                  & {\color[HTML]{3531FF} 0.0616} & {\color[HTML]{3531FF} 0.0364} & {\color[HTML]{3531FF} 0.0561} & {\color[HTML]{3531FF} 0.0653} & {\color[HTML]{3531FF} 0.0541} & {\color[HTML]{3531FF} 0.0521} \\ \hline
                                               & corr1                     & 0.1699                        & 0.1929                        & 0.1993                        & 0.2014                        & 0.2035                        & 0.2134                        \\
                                               & corr2                     & {\color[HTML]{009901} 0.1490} & {\color[HTML]{009901} 0.1386} & {\color[HTML]{009901} 0.1303} & {\color[HTML]{009901} 0.1118} & {\color[HTML]{009901} 0.1133} & {\color[HTML]{009901} 0.1188} \\
                                               & TS2VEC                    & 0.1897                        & 0.1975                        & 0.2151                        & 0.2074                        & 0.2013                        & 0.1871                        \\
\multirow{-4}{*}{SSE}                          & SimStock                  & {\color[HTML]{3531FF} 0.1106} & {\color[HTML]{3531FF} 0.0921} & {\color[HTML]{3531FF} 0.1128} & {\color[HTML]{3531FF} 0.1072} & {\color[HTML]{3531FF} 0.1074} & {\color[HTML]{3531FF} 0.1167} \\ \hline
                                               & corr1                     & 0.2248                        & 0.2183                        & 0.2123                        & 0.2156                        & 0.2106                        & 0.2042                        \\
                                               & corr2                     & {\color[HTML]{3531FF} 0.1103} & {\color[HTML]{009901} 0.1143} & {\color[HTML]{009901} 0.1164} & {\color[HTML]{009901} 0.1122} & {\color[HTML]{009901} 0.1212} & {\color[HTML]{009901} 0.1239} \\
                                               & TS2VEC                    & 0.1642                        & 0.1796                        & 0.1684                        & 0.1689                        & 0.1702                        & 0.1594                        \\
\multirow{-4}{*}{SZSE}                         & SimStock                  & {\color[HTML]{3531FF} 0.1103} & {\color[HTML]{3531FF} 0.1130} & {\color[HTML]{3531FF} 0.1157} & {\color[HTML]{3531FF} 0.1105} & {\color[HTML]{3531FF} 0.1047} & {\color[HTML]{3531FF} 0.1020} \\ \hline
                                               & corr1                     & 0.1308                        & 0.1363                        & 0.1239                        & 0.1429                        & 0.1450                        & 0.1472                        \\
                                               & corr2                     & {\color[HTML]{3531FF} 0.0723} & {\color[HTML]{009901} 0.0846} & {\color[HTML]{009901} 0.0762} & {\color[HTML]{009901} 0.0871} & {\color[HTML]{009901} 0.0818} & {\color[HTML]{009901} 0.0810} \\
                                               & TS2VEC                    & 0.1066                        & 0.1142                        & 0.1153                        & 0.1136                        & 0.1108                        & 0.1215                        \\
\multirow{-4}{*}{TSE}                          & SimStock                  & {\color[HTML]{009901} 0.0842} & {\color[HTML]{3531FF} 0.0703} & {\color[HTML]{3531FF} 0.0704} & {\color[HTML]{3531FF} 0.0640} & {\color[HTML]{3531FF} 0.0570} & {\color[HTML]{3531FF} 0.0625} \\ \hline
\end{tabular}
\end{table}

==> Tables/chap_4_pair_trading_top3_2021.tex <==
\useunder{\uline}{\ul}{}

\fontsize{7}{8}\selectfont{
\begin{tabular}{cccccc}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Query\\ Stock\end{tabular}}} & \multicolumn{5}{c}{\textbf{Wealth}}                                                                                                                                            \\
                                                                                & \textbf{SimStock}                 & \textbf{TS2VEC}               & \textbf{Corr1}                   & \textbf{Corr2}                     & \textbf{Coint}                     \\ \hline
AAPL                                                                            & 914.75 \tiny{$\pm$334.8}            & {\ul 1186.87 \tiny{$\pm$162.8}} & 725.72 \tiny{$\pm$677.9}           & 522.78 \tiny{$\pm$932.78}            & \textbf{1770.44 \tiny{$\pm$1770.44}} \\
CMG                                                                             & \textbf{581.0 \tiny{$\pm$808.77}}   & {\ul 279.23 \tiny{$\pm$405.03}} & -708.54 \tiny{$\pm$699.87}         & -1227.58 \tiny{$\pm$855.19}          & -1632.0 \tiny{$\pm$1470.72}          \\
MSFT                                                                            & \textbf{853.32 \tiny{$\pm$103.37}}  & 509.43 \tiny{$\pm$762.5}        & {\ul 511.9 \tiny{$\pm$981.73}}     & 255.29 \tiny{$\pm$1162.8}            & -1364.24 \tiny{$\pm$501.4}           \\
WFC                                                                             & \textbf{518.85 \tiny{$\pm$267.0}}   & 23.05 \tiny{$\pm$503.27}        & 17.66 \tiny{$\pm$497.41}           & 360.4 \tiny{$\pm$615.0}              & {\ul 437.66 \tiny{$\pm$384.22}}      \\
V                                                                               & {\ul 327.19 \tiny{$\pm$127.59}}     & 2.51 \tiny{$\pm$223.95}         & \textbf{338.82 \tiny{$\pm$101.38}} & -127.91 \tiny{$\pm$318.0}            & -377.59 \tiny{$\pm$429.87}           \\
XOM                                                                             & \textbf{322.59 \tiny{$\pm$1251.16}} & NaN                           & -336.94 \tiny{$\pm$562.32}         & {\ul 81.14 \tiny{$\pm$1131.77}}      & NaN                                \\
PFE                                                                             & 174.03 \tiny{$\pm$226.39}           & NaN                           & {\ul 384.26 \tiny{$\pm$1703.69}}   & 31.52 \tiny{$\pm$478.12}             & \textbf{1611.53 \tiny{$\pm$2858.75}} \\
AMZN                                                                            & {\ul 832.04 \tiny{$\pm$159.02}}     & 747.52 \tiny{$\pm$777.45}       & -921.59 \tiny{$\pm$758.14}         & \textbf{1395.02 \tiny{$\pm$2328.78}} & 474.59 \tiny{$\pm$3785.81}           \\
BA                                                                              & \textbf{580.68 \tiny{$\pm$2267.44}} & {\ul 113.48 \tiny{$\pm$703.2}}  & -1211.11 \tiny{$\pm$658.4}         & -1093.42 \tiny{$\pm$1597.89}         & -824.94 \tiny{$\pm$1637.36}          \\
META                                                                            & \textbf{3355.94 \tiny{$\pm$ NaN}}   & 483.08 \tiny{$\pm$ NaN}         & {\ul 2406.5 \tiny{$\pm$77.94}}     & -842.84 \tiny{$\pm$3966.82}          & NaN                                \\
MA                                                                              & {\ul 163.72 \tiny{$\pm$81.76}}      & -14.69 \tiny{$\pm$377.52}       & 281.05 \tiny{$\pm$73.06}           & 64.33 \tiny{$\pm$1345.97}            & \textbf{544.03 \tiny{$\pm$516.96}}   \\
CVS                                                                             & {\ul 914.14 \tiny{$\pm$497.59}}     & -320.82 \tiny{$\pm$336.81}      & 802.74 \tiny{$\pm$1221.49}         & \textbf{970.3 \tiny{$\pm$579.37}}    & -1079.35 \tiny{$\pm$2857.85}         \\ \hline
\end{tabular}}

==> Tables/chap_pair_trading_top3_mdd.tex <==
\begin{table}[]
\useunder{\uline}{\ul}{}
\fontsize{7}{8}\selectfont{
\begin{tabular}{cccccc}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Query\\ Stock\end{tabular}}} & \multicolumn{5}{c}{\textbf{Maximum Drawdown (\%)}}                                                                                                               \\
                                                                                & \textbf{SimStock}                   & \textbf{TS2VEC}               & \textbf{Corr1}                & \textbf{Corr2}                & \textbf{Coint}     \\ \hline
AAPL                                                                            & \textbf{-1.91 \tiny{$\pm$0.67}}       & $\text{NaN}^{**}$                            & -6.05 \tiny{$\pm$3.47}          & {\ul -3.4 \tiny{$\pm$2.00}}     & $\text{NaN}^{**}$                         \\
CMG                                                                             & \textbf{-2.98 \tiny{$\pm$2.54}}       & {\ul -6.37 \tiny{$\pm$2.22}}    & -14.96 \tiny{$\pm$6.38}         & -15.52 \tiny{$\pm$10.36}        & -20.03 \tiny{$\pm$15.47}     \\
MSFT                                                                            & \textbf{-3.79 \tiny{$\pm$0.21}}       & {\ul -5.66 \tiny{$\pm$0.24}}    & -7.12 \tiny{$\pm$4.72}           & -12.89 \tiny{$\pm$12.54}        & -13.23 \tiny{$\pm$2.96}      \\
WFC                                                                             & \textbf{-2.2 \tiny{$\pm$3.77}}        & -9.16 \tiny{$\pm$8.29}           & {\ul -5.75 \tiny{$\pm$4.53}}    & $\text{NaN}^{**}$                            & -23.95 \tiny{$\pm$13.75}     \\
V                                                                               & {\ul -2.22 \tiny{$\pm$2.55}}          & -2.38 \tiny{$\pm$2.77}          & \textbf{-0.43 \tiny{$\pm$0.75}} & -3.17 \tiny{$\pm$4.47}          & -7.46 \tiny{$\pm$5.87}       \\
XOM                                                                             & {\ul -3.38 \tiny{$\pm$0.44}}           & \textbf{-3.02 \tiny{$\pm$2.95}} & -4.71 \tiny{$\pm$1.42}          & -6.61 \tiny{$\pm$7.06}           & -9.29 \tiny{$\pm$7.58}        \\
PFE                                                                             & {\textbf{-7.84 \tiny{$\pm$7.41}}} & -10.03 \tiny{$\pm$13.49}         & -9.99 \tiny{$\pm$9.43}          & -10.43 \tiny{$\pm$5.06}         & {\ul -9.03 \tiny{$\pm$5.56}} \\
AMZN                                                                            & {\ul -5.05 \tiny{$\pm$4.99}}          & \textbf{-4.67 \tiny{$\pm$2.33}} & -15.12 \tiny{$\pm$9.38}         & -8.96 \tiny{$\pm$4.15}          & -31.90 \tiny{$\pm$13.12}     \\
BA                                                                              & {\ul -12.09 \tiny{$\pm$11.57}}         & \textbf{-5.87 \tiny{$\pm$2.13}} & -15.46 \tiny{$\pm$8.62}         & -12.86 \tiny{$\pm$3.26}         & -14.43 \tiny{$\pm$7.32}      \\
META                                                                            & \textbf{-4.91 \tiny{$\pm$$\text{NaN}^{*}$}}        & {\ul -8.75 \tiny{$\pm$8.98}}    & -11.58 \tiny{$\pm$4.95}         & -33.98 \tiny{$\pm$25.84}        & -25.40 \tiny{$\pm$11.24}     \\
MA                                                                              & \textbf{-2.18 \tiny{$\pm$2.51}}       & -5.01 \tiny{$\pm$5.19}           & {\ul -2.58 \tiny{$\pm$2.72}}    & -6.85 \tiny{$\pm$7.23}          & -11.51 \tiny{$\pm$4.66}      \\
CVS                                                                             & {\ul -3.01 \tiny{$\pm$1.84}}          & -9.08 \tiny{$\pm$8.32}           & -4.58 \tiny{$\pm$4.59}           & \textbf{-2.92 \tiny{$\pm$1.37}} & -19.85 \tiny{$\pm$17.02      \\ \hline

\end{tabular}}
\end{table}

==> Tables/chap_pair_trading_top3_mdd_2022.tex <==

\fontsize{7}{8}\selectfont{
\begin{tabular}{cccccc}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Query\\ Stock\end{tabular}}} & \multicolumn{5}{c}{\textbf{Maximum Drawdown (\%)}}                                                                                                                    \\
                                                                                & \textbf{SimStock}             & \textbf{TS2VEC}               & \textbf{Corr1}                & \textbf{Corr2}                & \textbf{Coint}         \\ \hline
AAPL                                                                            & \textbf{-2.58 \tiny{$\pm$0.47}} & -3.57 \tiny{$\pm$2.7}           & {\ul -3.4 \tiny{$\pm$1.43}}     & -4.81 \tiny{$\pm$5.95}          & -9.46 \tiny{$\pm$9.46}   \\
CMG                                                                             & \textbf{-3.47 \tiny{$\pm$2.38}} & {\ul -4.12 \tiny{$\pm$2.86}}    & -11.66 \tiny{$\pm$5.64}         & -15.54 \tiny{$\pm$10.74}        & -21.93 \tiny{$\pm$9.63}  \\
MSFT                                                                            & \textbf{-2.02 \tiny{$\pm$1.63}} & -5.76 \tiny{$\pm$0.29}          & {\ul -4.65 \tiny{$\pm$4.28}}    & -11.21 \tiny{$\pm$9.59}         & -18.99 \tiny{$\pm$4.65}  \\
WFC                                                                             & {\ul -3.97 \tiny{$\pm$3.46}}    & -4.65 \tiny{$\pm$1.63}          & -8.16 \tiny{$\pm$3.01}          & \textbf{-3.26 \tiny{$\pm$3.08}} & -11.14 \tiny{$\pm$3.05}  \\
V                                                                               & {\ul -2.08 \tiny{$\pm$2.61}}    & -2.33 \tiny{$\pm$2.8}           & \textbf{-0.47 \tiny{$\pm$0.81}} & -6.41 \tiny{$\pm$5.77}          & -10.06 \tiny{$\pm$0.63}  \\
XOM                                                                             & \textbf{-6.07 \tiny{$\pm$4.63}} & NaN                           & -8.01 \tiny{$\pm$2.96}          & {\ul -6.44 \tiny{$\pm$6.77}}    & NaN                    \\
PFE                                                                             & \textbf{-5.13 \tiny{$\pm$1.04}} & NaN                           & -7.2 \tiny{$\pm$10.88}          & {\ul -5.7 \tiny{$\pm$3.36}}     & -20.54 \tiny{$\pm$9.38}  \\
AMZN                                                                            & {\ul -3.79 \tiny{$\pm$3.28}}    & \textbf{-1.64 \tiny{$\pm$2.83}} & -17.46 \tiny{$\pm$5.79}         & -8.6 \tiny{$\pm$7.72}           & -19.78 \tiny{$\pm$13.31} \\
BA                                                                              & {\ul -11.83 \tiny{$\pm$11.76}}  & \textbf{-8.38 \tiny{$\pm$5.97}} & -15.48 \tiny{$\pm$8.63}         & -13.56 \tiny{$\pm$8.05}         & -22.8 \tiny{$\pm$18.89}  \\
META                                                                            & \textbf{-1.51 \tiny{$\pm$ NaN}} & {\ul -5.62 \tiny{$\pm$ NaN}}    & -17.84 \tiny{$\pm$8.65}         & -28.43 \tiny{$\pm$30.23}        & NaN                    \\
MA                                                                              & {\ul -2.7 \tiny{$\pm$2.5}}      & \textbf{-2.04 \tiny{$\pm$1.94}} & -2.54 \tiny{$\pm$2.73}          & -8.49 \tiny{$\pm$7.54}          & -4.22 \tiny{$\pm$1.24}   \\
CVS                                                                             & \textbf{-4.7 \tiny{$\pm$3.03}}  & -6.01 \tiny{$\pm$3.27}          & {\ul -5.65 \tiny{$\pm$4.04}}    & -5.67 \tiny{$\pm$3.75}          & -23.53 \tiny{$\pm$17.64} \\ \hline
\end{tabular}}
